ScaRR: Scalable Runtime Remote Attestation for Complex Systems

The introduction of remote attestation (RA) schemes has allowed academia and industry to enhance the security of their systems. The commercial products currently available enable only the validation of static properties, such as applications fingerprint, and do not handle runtime properties, such as control-flow correctness. This limitation pushed researchers towards the identification of new approaches, called runtime RA. However, those mainly work on embedded devices, which share very few common features with complex systems, such as virtual machines in a cloud. A naive deployment of runtime RA schemes for embedded devices on complex systems faces scalability problems, such as the representation of complex control-flows or slow verification phase. In this work, we present ScaRR: the first Scalable Runtime Remote attestation schema for complex systems. Thanks to its novel control-flow model, ScaRR enables the deployment of runtime RA on any application regardless of its complexity, by also achieving good performance. We implemented ScaRR and tested it on the benchmark suite SPEC CPU 2017. We show that ScaRR can validate on average 2M control-flow events per second, definitely outperforming existing solutions.

==> miscellaneous.tex <==
\section{Miscellaneous}

\textbf{THIS IS A DUMMY SECTION FOR DUMPING STUFFS}

Current control flow integrity checkers spend efforts in adding checkers within the application code. This is achieved by using instrumentation at compilation time, at system level, or at hardware level. The main point of these approaches is that the program checks whether its next jump (or call) location is valid or not. In this setting, all attacks are aimed to corrupt the program and the checking system because both lean in the same memory region.
With this approach, we aim to change this paradigm (need to check how much innovative is) by moving the control flow verification inside external libraries. In this way, even if an attacker can perform memory corruption attacks into the program, the library can recognize an unforeseen behavior at the caller side.

\paragraph{\textbf{Approach}} \textbf{1)} We want to identify anomalous CFG without generating all possible combinations. 
\textbf{2)} An attack against CFG is acceptable as long as it does not reach te OS through some shared library.

\subsection{Contributions}
\begin{itemize}
	\item Make a scalable graph model for large program
	\item Deal with ASLR
	\item Shared library
	\item Handing exception (probably)
\end{itemize}

\subsection{Challenges}
This setting implies a set of challenges to overcome:
\begin{itemize}
	\item We have to define the list of valid application status.
	\item We have to update application status at runtime without editing the original program.
	\item The entire system should be more efficient than classic shadow stack solutions. And maybe more robust, or more light, or more something.
\end{itemize}

\subsection{Solutions}
\begin{itemize}
	\item Static analysis of the code. using angr
	\item Instrumentation, pin tool will do.
	\item Cumulative hash, at this purpose we should find a way for reducing call graph space in a cool manner. Maybe getting inspiration from CFG. We can use BLAKE-2, a fast-cumulative hash function. TODO: find a good modeling of call graph
\end{itemize}

\subsection{Interesting points}
Without any sorting
\begin{itemize}
	\item I am interested to CALL and RET instructions, not to the entire control-flow graph.
	\item As ``node'' labels, we can use relative address of instructions + all possible destinations of that call.
	\item I don’t care if the program is messed up internally by some rop attack or memory corruption attack. I need only to verify that its status is correct once the control leaves the application.
	\item ROP chains, return address override, and function pointers override are based on CALL and RET instruction, which look called strangely during the attack. Therefore, from my point of view, it is enough to trace them.
	\item Data oriented attacks are different, maybe we can include them too.
	\item Security checks are performed at library level because I want to check the program status once it tries to communicate with the rest of the system.
	\item This system can be seen as an attestation among entities within the same machine (dynamic local attestation?) IMPORTANT: discuss with Mauro, this work looks very similar to this paper “C-FLAT: Control-Flow Attestation for Embedded Systems Software”@ccs2016
	\item I have to identify the entry points of external libraries. Then for each entry point I list its ``valid application status''. It is not just a general list of valid status like in C-FLAT.
\end{itemize}

\subsection{Strong points}
\begin{itemize}
	\item First propose of local dynamic attestation (maybe Microsoft did something similar, but less good)
	\item We propose a better analysis, and a better status modeling. Recursions, do you remember them?
	\item Better performances, we check only once control lease program
\end{itemize}

Some consideration

\subsection{Stuff to discuss somewhere}

\begin{itemize}
	\item Load the library with a signature, the process has to be sure the library is trusted as well - you can use a static signature from SGX
	\item How to make a full control flow graph: find a better analyzer (this is not the case), try a combination of dynamic analysis and static (I prefer this), develop an our technique (this is out of cope I guess)
	\item \textbf{WHY DO YOU NEED SGX FOR THIS?!}
\end{itemize}

The overview of the system is formed by 3 entities:
\begin{description}
	\item[Application] it is the program we intend to protect.
	\item[External libraries] system libraries which allow an application to communicate with the rest of the system.
	\item[Verification system] a verification system, implemented with trusted computing techniques, which validates the interaction between application and libraries.
\end{description}

In the above picture, it is possible to see how the 3 entities work together. The application still updates its status, which is stored in a dedicated memory region (tc). Once the application calls a library function, the latter queries the verifier in order to compare the application status with all valid application status.

\subsection{Control Flow Graph Model}

How do we model a control flow graph? And why in this way?

\textbf{MAIN IDEA} every edge which enters in a function, must return in the same function of before, \ie link call to a function with the respective return

\begin{figure}[t]
	\centering
	\includegraphics[width=0.5\textwidth]{fig/time-evolving}
	\caption{Example of time evolution of a program\todo{FT: make a better image!}}
	\label{fig:time-evolving}
\end{figure}

Figure~\ref{fig:time-evolving} descries a function calls and return operations in a general application.

\begin{algorithm}
	\caption{My algorithm}\label{euclid}
	\begin{algorithmic}[1]
		\Procedure{main}{}
		\State a()
		\EndProcedure
		\Procedure{a}{}
		\State fn1()
		\State b()
		\EndProcedure
		\Procedure{b}{}
		\State fn2()
		\EndProcedure
	\end{algorithmic}
\end{algorithm}

\begin{figure*}[t]
	\centering
	\includegraphics[width=\textwidth]{fig/cfg-not-optimized}
	\caption{Example of CFG not optimized\todo{FT: make a better image!}}
	\label{fig:cfg-not-optimized}
\end{figure*}

Figure~\ref{fig:cfg-not-optimized} shows an example of a CFG not optimized, each external function (\ie red nodes) is linked by each possible path. This might bring to an explosion of combinations.

\begin{figure*}[t]
	\centering
	\includegraphics[width=\textwidth]{fig/cfg-optimized}
	\caption{Example of CFG optimized\todo{FT: make a better image!}}
	\label{fig:cfg-optimized}
\end{figure*}

Figure~\ref{fig:cfg-optimized} shows an example of a CFG optimized, each external function (\ie red nodes) is linked an abstract edge which contains the properties required to validate paths between two nodes. This limits path explosion.
